Reinforcement Learning with Dynamic Convex Risk Measures

We develop an approach for solving time-consistent risk-sensitive stochastic optimization problems using model-free reinforcement learning (RL). Specifically, we assume agents assess the risk of a sequence of random variables using dynamic convex risk measures. We employ a time-consistent dynamic programming principle to determine the value of a particular policy, and develop policy gradient update rules that aid in obtaining optimal policies. We further develop an actor-critic style algorithm using neural networks to optimize over policies. Finally, we demonstrate the performance and flexibility of our approach by applying it to three optimization problems: statistical arbitrage trading strategies, financial hedging, and obstacle avoidance robot control.

==> section-files/estimate-value.tex <==
%!TEX root = ../main.tex

% --------------------------------------------------------------
%                         Estimation of the value function
% --------------------------------------------------------------
\subsection{Value Function Estimation}
\label{ssec:estimate-value}

The value function 
%$\valuefunc_{\timeidx}(\state; \policyparams)$ 
$\valuefunc^\phi$
may be estimated by using the recursion in \cref{eq:value-func1,eq:value-func2}.
We use the simulation upon simulation approach mentioned previously.
More precisely, when sampling a certain state $\state_{\timeidx}$, we also generate $\Ntransitions$ (inner) \transitionnames{} from the \stratname{} $\policy^{\policyparams}$ to obtain the tuples $(\state_{\timeidx}, \action_{\timeidx}^{(\transitionidx)}, \state_{\timeidx+1}^{(\transitionidx)}, \costfunc_{\timeidx}^{(\transitionidx)})$, $\transitionidx=1,\ldots,\Ntransitions$.
We can then estimate the one-step conditional risk measures for any given state using those additional \transitionnames{}.
To update the value function, we perform this simulation process for a mini-batch of states, compute the predicted (i.e. output of $\valuefunc^{\valueparams}$) and target values (i.e. \cref{eq:value-func1,eq:value-func2}), and calculate the expected square loss between these values.
We update the parameters using the Adam optimizer \citep{kingma2014adam} and repeat this process for several epochs in order to provide a good approximation of the value function.
We recall that the policy $\policy^{\policyparams}$ is fixed while we optimize $\valuefunc^{\valueparams}$.
The algorithm is provided in \cref{algo:estimate-value}.
\input{section-files/figures-algo-updateV}

A powerful result for neural networks structures is the \emph{universal approximation theorem} -- see e.g. \cite{cybenko1989approximation,hornik1991approximation,leshno1993multilayer,pinkus1999approximation}.
\begin{theorem}[Universal Approximation \citep{cybenko1989approximation}]
    \label{thm:universal-approx}
    Let $d_1, d_2\in \Nats$ and $\sigma$ be an activation function.
    Then $\sigma$ is not a polynomial iff for any continuous function $f:\Reals^{d_1} \rightarrow \Reals^{d_2}$, any compact subset $K \subset \Reals^{d_1}$ and any $\epsilon > 0$, there exists a neural network $\hat{f}_{\epsilon}:\Reals^{d_1} \rightarrow \Reals^{d_2}$ with representation $\hat{f}_{\epsilon} = W_2 \circ \sigma \circ W_1$ such that $\sup_{x \in K} \norm[0]{ f(x) - \hat{f}_{\epsilon}(x) } < \epsilon$. 
\end{theorem}

We prove next that for a fixed \stratname{} $\policy^{\policyparams}$, we can approximate its corresponding value function $\valuefunc_{\timeidx}(\state; \policyparams)$ with an \ANN{} using the procedure devised in \cref{algo:estimate-value}.
\cref{thm:approx-valuefunc} follows from the universal approximation theorem.
\begin{theorem}[Approximation of $\valuefunc$]
    \label{thm:approx-valuefunc}
    %Consider the framework devised in \cref{sec:problem-setup} with the value function $\valuefunc$ defined in \cref{eq:value-func}.
    Let $\policy^{\policyparams}$ denote a fixed \stratname{}, with corresponding value function as defined in \cref{eq:value-func}, which we denote $\valuefunc_{\timeidx}(\state; \policyparams)$.
    Then for any $\epsilon^{*} > 0$, there exists an \new{\ANN{}} $\valuefunc_{\timeidx}^{\valueparams}: \statespace \rightarrow \Reals$ such that $\esssup_{\state \in \statespace} \norm[0]{ \valuefunc_{\timeidx}(\state; \policyparams) - \valuefunc_{\timeidx}^{\valueparams}(\state; \policyparams) } < \epsilon^{*}$, for any $\timeidx \in \periodspace$.
\end{theorem}

\begin{proof}[Proof of \cref{thm:approx-valuefunc}]
First, we prove a lemma that states convex risk measures are \new{absolutely} continuous since they are in fact monetary.
\new{In what follows, the norm is to be understood as the $\infty$-norm.}
%This comes in handy when dealing with the universal approximation theorem.
\begin{lemma}
    \label{lemma:continuity}
    \new{Monetary} one-step conditional risk measures $\riskmeas_{\timeidx}$ are absolutely continuous a.s..
\end{lemma}
\begin{proof}[Proof of \cref{lemma:continuity}]
    Indeed, starting from the inequality $\randvar \leq \randvardum + \norm{ \randvar - \randvardum }$, where $\randvar,\randvardum \in \Lpspace_{\timeidx+1}$, and using the monotonicity and translation invariance properties, we have
    \begin{equation}
        \riskmeas_{\timeidx}(\randvar) \leq \riskmeas_{\timeidx}(\randvardum + \norm{\randvar-\randvardum}) \implies \riskmeas_{\timeidx}(\randvar) - \riskmeas_{\timeidx}(\randvardum) \leq \norm{\randvar - \randvardum}.
    \end{equation}
    Repeating this with $\randvardum \leq \randvar + \norm{\randvar-\randvardum}$ yields to 
    \begin{equation}
        \esssup \norm{\riskmeas_{\timeidx}(\randvar) - \riskmeas_{\timeidx}(\randvardum)} \, \leq \norm{\randvar-\randvardum}.
    \end{equation}
    Therefore convex risk measures are Lipschitz continuous a.s. wrt the essential supremum norm, and hence they are absolutely continuous a.s..
\end{proof}
Next, recall that the value function given in \cref{eq:value-func} is a dynamic convex risk measure, and therefore may be written recursively with the \DPE{} in \cref{eq:value-func0-1,eq:value-func0-2} as
\begin{equation}
    \valuefunc_{\timeidx}(\state;\policyparams) =
    \riskmeas_{\timeidx} \Big(\costfunc_{\timeidx}^{\policyparams} +
    \valuefunc_{\timeidx+1}(\state_{\timeidx+1}^{\policyparams};\policyparams)
    \Bigm|\state_{\timeidx}=\state \Big).
\end{equation}

\new{We prove that the \ANN{} $\valueparams$ approximate the value function by induction.}
Without loss of generality, let us consider the case where the first dimension of the state space $\statespace$ corresponds to the time $\timeidx \in \periodspace$.
At the \timename{} $\eplength-1$, we have that
\begin{equation}
    \valuefunc_{\eplength-1}(\state;\policyparams) =
    \riskmeas_{\eplength-1} \Big(\costfunc_{\eplength-1}^{\policyparams} \Bigm|\state_{\eplength-1}=\state \Big).
\end{equation}
This is a convex risk measure which is absolutely continuous a.s. by \cref{lemma:continuity}.
Using the universal approximation theorem given in \cref{thm:universal-approx}, we obtain that \new{for any $\epsilon_{\eplength-1}>0$,} there exists a neural net $\phi$ such that
\begin{equation}
    \esssup_{\state \in \statespace} \norm{ \valuefunc_{\eplength-1}(\state; \policyparams) - \valuefunc_{\eplength-1}^{\valueparams}(\state; \policyparams) } < \epsilon_{\eplength-1}.
    \label{eq:induction-base}
\end{equation}
\new{This proves the base case of our proof by induction.}


For \new{the induction step}, the \ANN{} \new{$\valueparams$} approximates the value function at \timename{} $\timeidx$ as long as the value function at the next \timename{} $\timeidx+1$ is adequately approximated.
\new{Assume that for any $\epsilon_{\timeidx+1} > 0$, there exists an \ANN{} such that
\begin{equation}
    \esssup_{\state \in \statespace} \norm{ \valuefunc_{\timeidx+1}(\state; \policyparams) - \valuefunc_{\timeidx+1}^{\valueparams}(\state; \policyparams) } < \epsilon_{\timeidx+1}.\label{eq:induction-step}
\end{equation}}
Using the translation invariance, \new{the triangle inequality, \cref{lemma:continuity} and \cref{eq:induction-step}}, we have
\new{\begin{align}
    &\esssup_{\state \in \statespace} \norm{ \valuefunc_{\timeidx}(\state; \policyparams) - \valuefunc_{\timeidx}^{\valueparams}(\state; \policyparams) } \nonumber\\
    &\quad= \esssup_{\state \in \statespace} \norm{ \riskmeas_{\timeidx}\Big( \costfunc_{\timeidx}^{\policyparams} + \valuefunc_{\timeidx+1}(\state_{\timeidx+1}^{\policyparams}; \policyparams) \Bigm| \state_{\timeidx} = \state \Big)- \valuefunc_{\timeidx}^{\valueparams}(\state; \policyparams) } \nonumber\\
    &\quad\leq \esssup_{\state \in \statespace} \norm{ \riskmeas_{\timeidx}\Big( \costfunc_{\timeidx} + \valuefunc^{\valueparams}_{\timeidx+1}(\state_{\timeidx+1}^{\policyparams}; \policyparams) \Bigm| \state_{\timeidx} = \state \Big)- \valuefunc_{\timeidx}^{\valueparams}(\state; \policyparams) } \nonumber\\
    &\qquad\quad + \esssup_{\state \in \statespace} \norm{ \riskmeas_{\timeidx}\Big( \costfunc_{\timeidx}^{\policyparams} + \valuefunc_{\timeidx+1}(\state_{\timeidx+1}^{\policyparams}; \policyparams) \Bigm| \state_{\timeidx} = \state \Big)- \riskmeas_{\timeidx}\Big( \costfunc_{\timeidx} + \valuefunc^{\valueparams}_{\timeidx+1}(\state_{\timeidx+1}^{\policyparams}; \policyparams) \Bigm| \state_{\timeidx} = \state \Big) } \nonumber\\
    &\quad\leq \esssup_{\state \in \statespace} \norm{ \riskmeas_{\timeidx}\Big( \costfunc_{\timeidx} + \valuefunc^{\valueparams}_{\timeidx+1}(\state_{\timeidx+1}^{\policyparams}; \policyparams) \Bigm| \state_{\timeidx} = \state \Big)- \valuefunc_{\timeidx}^{\valueparams}(\state; \policyparams) } \nonumber\\
    &\qquad\quad + \esssup_{\state \in \statespace} \norm{  \valuefunc_{\timeidx+1}(\state; \policyparams) -  \valuefunc^{\valueparams}_{\timeidx+1}(\state; \policyparams) } \nonumber\\ 
    &\quad< \esssup_{\state \in \statespace} \norm{ \riskmeas_{\timeidx}\Big( \costfunc_{\timeidx} + \valuefunc^{\valueparams}_{\timeidx+1}(\state_{\timeidx+1}^{\policyparams}; \policyparams) \Bigm| \state_{\timeidx} = \state \Big) - \valuefunc_{\timeidx}^{\valueparams}(\state; \policyparams) } + \epsilon_{\timeidx+1}. \label{eq:proof-induction1}
    %&\quad< \epsilon_{\timeidx} + \epsilon_{\timeidx+1}. \nonumber 
\end{align}Using the universal approximation theorem on \cref{eq:proof-induction1}, we get for any $\epsilon_{\timeidx}>0$ that
\begin{equation}
    \esssup_{\state \in \statespace} \norm{ \valuefunc_{\timeidx}(\state; \policyparams) - \valuefunc_{\timeidx}^{\valueparams}(\state; \policyparams) } < \epsilon_{\timeidx} + \epsilon_{\timeidx+1}
\end{equation}We apply this argument recursively for any \timename{} $\timeidx \in \periodspace$, which completes the proof by induction.}
As \cref{thm:universal-approx} is valid for any $\epsilon>0$, we can perform the training procedure in order to construct a sequence of $\epsilon_{\timeidx}, \ \timeidx \in \periodspace$ that satisfies a global error $\epsilon^{*}$, such as $\sum \epsilon_{\timeidx} < \epsilon^{*}$.
\end{proof}
